Comparative Analysis of Change Blindness in Virtual Reality and Augmented Reality Environments

Change blindness is a phenomenon where an individual fails to notice alterations in a visual scene when a change occurs during a brief interruption or distraction. Understanding this phenomenon is specifically important for the technique that uses a visual stimulus, such as Virtual Reality (VR) or Augmented Reality (AR). Previous research had primarily focused on 2D environments or conducted limited controlled experiments in 3D immersive environments. In this paper, we design and conduct two formal user experiments to investigate the effects of different visual attention-disrupting conditions (Flickering and Head-Turning) and object alternative conditions (Removal, Color Alteration, and Size Alteration) on change blindness detection in VR and AR environments. Our results reveal that participants detected changes more quickly and had a higher detection rate with Flickering compared to Head-Turning. Furthermore, they spent less time detecting changes when an object disappeared compared to changes in color or size. Additionally, we provide a comparison of the results between VR and AR environments.

==> Contents/Discussion_AdditionalWriting.tex <==


\section{Discussion}
% The results of our two user studies provide insights into the participants' performance and perception in different experimental conditions in VR and AR. 
The two user studies in VR and AR provide insights into the participants' performance and perception. In this section, we discuss our findings and compare the results between VR and AR.

% \subsection{
\paragraph{\textbf{Detection Time}}
% ----------- RQ - 1: FoV, VR / AR
The participants demonstrate faster detection of the altered object in the Flickering condition compared to the Head-Turning condition in both VR and AR. This result represents that when object alternation has occurred outside of FoV, it takes more time for participants to detect the changes compared to when it occurred within FoV. The participants' comments also support this, as they mentioned difficulties in paying attention to the objects when the objects moved out of the FoV.
This finding supports H1 that the participants would spend more time turning their heads and refocusing the scene leading the slower detection in the Head-Turning condition.
% Interestingly, in AR, there was no significant difference in detection time between the two different head-turning conditions, which rejects H3.

% this could be a limitation, we only 
In the AR experiment, different angles of the Head-Turning conditions do not affect the participants' detection time.
%This result shows that the change detection speed is not affected by how long the altered object was outside of the FoV. 
This also indicates that the narrower FoV does not significantly impact the detection of changes occurring outside of the FoV.
This rejects H4. However, it would be affected if the altered object remains outside of the FoV significantly longer period than just during the Head-Turning.
Further studies are needed to evaluate the effect of the significantly long period when the altered object is out of the FoV.
% that a larger angle with the head-turning condition has a worse effect on the change detection.


% ----------- RQ - 2: Alternation conditions
Regarding the object alteration conditions, our findings in both VR and AR align with the previous studies conducted in a 2D environment\cite{rensink1997see,ma2013change}.
% However, it contrasts with the recent study conducted in a VR environment, which reported no significant effect between the object alternation conditions \cite{martin2023study}.
% However, it contrasts with the recent study conducted in a VR environment \cite{martin2023study}.
With the Removal condition, the detection time is significantly faster than the result with the Color Alteration, Size Incrementation, and Decrementation conditions in both VR and AR.
This finding supports H2 that the participants would find the altered object with the Removal condition easily. 

% In the AR environment, the result shows that the detection time with the removal condition is also significantly faster than the result with other conditions.
In AR, however, the result with the Color Alteration condition is significantly slower than the result with the Removal condition and size alteration conditions.
Interestingly, the increase in detection time with the Color Alternation condition in AR is only 5.76\% compared to VR, while the other conditions show increases of at least 24.0\% and up to 28\%.
This result suggests that the perception of the color visual channel is not significantly decreased in AR compared to VR. This supports H3, that the visual channel would be perceived differently in AR and VR.
Additionally, this result aligns with the conventional approach of visual perception (i.e., the coherence theory and triadic architecture) \cite{rensink2000visual,rensink2002change} which proposes each visual channel is perceived differently. Consequently, these detection time results represent that the limited FoV and type of visual channel influence how fast the observer can detect changes.


The 3-way mixed ANOVA (2 immersive environment x 2 visual attention-disturbing \footnote{For the mixed ANOVA, we only include the 60$^\circ$ Head-Turning from the AR study.} x 3 object alteration) shows a main effect on the detection time of the immersive environment (F(1, 42)=5.051, $p$=.030, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.107). However, no interaction effect is found related to the immersive environment. Overall, the average detection time in the VR environment (M=15.33s, SD=6.41) is significantly faster than the one in the AR environment (M=17.74s, SD=8.33).
This difference can be because of the different sizes of the FoV and different environmental characteristics, such as different object transparency in VR and AR environments.
% Overall, the participants in VR exhibited faster detection times compared to participants in the AR condition.
% The absence of interaction effects related to the immersive technologies suggests that the limitations of the AR headset have a significant impact on overall performance in detecting changes in the virtual scene.

% RQ - 1: FoV
% The alternation that occurred inside or outside of the FoV affects the change detection regardless of the type of immersive environment.
%it is a consistent result with the previous change blindness study in VR \cite{martin2023study}.
% But interestingly, how long the altered object is out of the FoV does not affect the change detection.
% According to this result and the comments from the participants, in which they could not have attention well to the objects when the object moved out of the FoV, how long the altered object is out of the FoV does not meaningful for the change detection.

% RQ - 1: VR / AR
% The average detection time result in the VR environment (M=15.33s, SD=6.41) is significantly faster than the result in the AR environment (M=17.74s, SD=8.33) (F(1, 42)=5.051, $p$=.030, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.107).
% This difference can be due to a different size of FoV or different environmental characteristics, such as object transparency.

% According to the comments from the participants, they could not have attention well on the objects when they were moved out of the FoV.

% RQ - 2
% The results with object alternation conditions present that how the object changed is essential to understanding change blindness.
% This result supports the conventional approach of visual perception (coherence theory and triadic architecture) \cite{rensink2000visual,rensink2002change}, which proposes each visual channel is perceived differently, but it is in contrast with the previous change blindness study in the VR environment \cite{martin2023study}.

% This is the finding strategy
%In both VR and AR environments, the altered object on the 4th (top) and 3rd shelves was found faster than the object on the 2nd and 1st shelves. Interestingly, the detection time result with the altered object on the 2nd shelf was faster than the object on the 1st shelf only in the VR environment. We guess that difference occurred by the difference in FoV between the VR and AR devices. In the VR experiment, the participants could see the entire object at once, but they could only see objects on two shelves in the AR experiment (Figure~\ref{figure:FoV} shows this FoV difference).
%But from the qualitative questionnaire result, participants generally used the finding strategy of the altered object from top to bottom and row by row. Consequently, participants could find the altered object from top to bottom without a gaze height shifting in VR.  However, they should change the gaze height in AR to see objects on other shelves. We guess that the FoV limitation and the participants' common strategy made shelves in two groups: upper and lower shelves in AR, and we guess it is the cause of the different detection times with the location of the altered object. This result supports H6, the detection time difference as the participant's finding strategy affects the altered object location.

% This is the finding strategy end

% However, it is important to note that the narrow FoV may still affect overall perception by increasing the likelihood of altered objects being outside of the participants' visual range.

% \dhk{With the flicker method, the participants can see the original object and altered object within just one second (original object (250ms), sight-blocking (250ms), altered object (250ms), sight-blocking (250ms). However, they could find the object almost after 12 seconds even though they already knew that one object would be changed.
% Consequently, this result represents that our VR environment and the tasks well occurred the change blindness phenomenon.}

% \dhk{At first, with the flickering method, participants could find the manipulated object faster than with the turning-60\textdegree method.
% It could be because the participants could focus on the same location easily with the flickering method.}

% \dhk{Second, when the object is removed, participants can find it faster than when its color or size is changed.
% According to the coherence theory and triadic architecture \cite{rensink2002change, rensink2000dynamic}, the spatial information is stored in the working memory. Even though its capacity is limited, working memory is a rapidly storable system that can handle a visual change \cite{chatham2015multiple}.
% Thus, we guess because of the spatial information of objects being stored easily and rapidly, participants could find the removed object faster than changing its color or size.}

% \dhk{Third, when the manipulated object is located higher floor, participants could find it faster than it was on the lower floor.
% In the questionnaire, participants answered they searched the changed object from top to bottom and floor by floor. Thus, this result represents that participants generally used this strategy.}

% \dhk{But interestingly, the object's basic color (Red, Green, Blue) does not affect the response time significantly. We guess that is because the color contrasts between the object's colors and the gray background are not significantly different. According to WCAG (Web Content Accessibility Guidelines), a recommended color contrast ratio is at least 3:1 for graphics. However, the color contrasts between them are 1.23:1 (Red), 2.35:1 (Green), and 2.65:1 (Blue).}

% \dhk{The flickering method resulted in a faster response time than the turning method regardless of the angles.
% The reason for the difference between the flickering and turning methods can be the same as the VR experiment result: the participant could focus on the same location easily.
% These results, non-difference results between the turning angles, represent that if the object is going out of the FoV, it affects the change detection, but the distance after the object goes out does not affect it.}

% \dhk{The object-manipulation method results show the removal method makes a faster response, likely the VR experiment. However, in this AR experiment, the Color change method made a faster response time than the size change methods.
% All other methods' response time results are increased by 24\% ~ 29\% from the VR experiment, but the color change method is only 5.7\%.
% This result can represent the color perception in AR environment is not too much weaker than in VR environment.}

% \dhk{The manipulated object's position effect is similar to the VR experiment, but one thing is different.
% When the object is located on the 4th and 3rd floor, it makes a faster response than it is on the 2nd and 1st floor.
% However, in the VR experiment, the object on the 2nd floor had a faster result than the 1st floor, but in the AR experiment, it could not.
% We guess the reason for this difference is the vertical FoV difference between the VR device and the AR device.
% The vertical FoV of the Vive Pro eye is \textcolor{red}{larger than 100\textdegree}, and it is enough FoV to see all floors at once, but the Hololends 2's vertical Fov is 29\textdegree; it can provide only \textcolor{red}{two} floors at once.
% Because of this different number of floors, the participant can see at once, we guess the object position-dependent response time result is different, even though they used the same strategy for both experiments.
% % The sight-blocking method and object-manipulation method both have a significant effect on the response time.
% % Their interaction is not statistically significant, but it shows more interaction than the VR study ($p$=.793 - VR; $p$=.082 - AR).
% % However, the mean response times are increased for each manipulation method (Removal: 11.87s -> 15.31s; Color: 17.25s -> 17.69s; Size: 16.89s -> 20.08s for increase, 17.74s -> 21.13s for decrease) compared with the VR study. But the increasing rate for the color manipulation case is significantly smaller than others. It could due to the transparency of the objects on the AR device.
% }

\paragraph{\textbf{Detection Rate}}
This detection rate results indicate which condition is more likely to cause confusion for the observer in change detection.
% ----------- RQ - 1: FoV, VR / AR
In the VR environment, an interaction effect is observed between the visual attention-disturbing and the object alteration conditions.
In the Head-Turning condition, the Removal condition's detection rate is higher than the results of the Size Incrementation and Decrementation conditions.
This indicates that the size alternation conditions can lead to confusion during change detection when combined with the Head-Turning condition, especially when the observer cannot maintain focus on the same location.
This finding supports H1 and H2, indicating that when moving the object out of the FoV can cause confusion for each visual channel differently.

% ----------- RQ - 2: Alternation conditions
In both immersive environments, the Removal condition has higher detection rates than the Size Incrementation and Decrementation.
The result of the Color Alteration condition is significantly less than the result of the Removal condition in VR, but it is significantly higher than the results with the size alternation conditions in AR.
This supports H1 and suggests that the color perception in both immersive environments is not significantly different.


The mixed ANOVA does not reveal a significant main effect on the detection rate between VR and AR. %The average detection rate result in the VR and AR experiments does not show a significant difference.
This suggests that, despite potential differences in visual perception speed between VR and AR, the accuracy of perception remains similar in both VR and AR. 
% This effect suggests that when the object is moved out from FoV, it causes confusion related to the volatility of the visual working memory, supporting H1 and H3.


% RQ - 1
% RQ - 2
% Interestingly, different from the detection time case, the result with the color alteration condition is not significantly different from the result with the removal condition.
% Similar to the environment cases, we can guess that even though the color visual channel is not good to perceive rapidly, visual confusion does not occur as much as the size alternations.


% However, no statistical differences are found among object alteration conditions in the head-turning condition.


% In addition, in the size decrementation and size incrementation conditions, flickering yielded higher accuracy compared to head-turning.
% However, no significant differences are observed between flickering and head-turning in the object removal and color alteration conditions.


% Overall, the detection rate of flickering is significantly higher than head-turning, and removal is more accurate than color alteration, size incrementation, and size decrementation.
% The results are consistent with the detection time result where conditions that cause confusion resulted in longer detection times.
% This suggests that participants selected the altered object after they had more certainty, indicating that detection time and rate can be indicators of change blindness.

% In AR, there is no significant difference in detection rates between flickering and the two head-turning conditions, while there is a main effect on the object alteration condition.
% Object removal and color alteration have a higher detection rate compared to size incrementation and decrementation conditions.
% Additionally, color change has a higher detection rate compared to both size alteration conditions.
% However, no significant difference was observed in detection rates between object removal and color alteration conditions.
% Flickering and 60$^\circ$ head-turning significantly differ in detection rates ($p$=.021), which is consistent with other results.
% However, the 30$^\circ$ head-turning condition is not significantly different from both other conditions, and the average rate is between those two conditions.
% We guess that this 30$^\circ$ head-turning condition's result indicates the longer time of cannot focusing on the objects enhances confusion, and this can support H1.
% In contrast with the detection time result, the detection rate results do not have a significant difference between AR and VR.

% Consequently, this detection rate results represent which condition makes the observer will have more confusion about the change detection.
% % RQ - 1
% Similar to the detection time results, the alteration that occurred outside of FoV makes an observer has a confusion about change detection.
% However, the immersive environment types do not affect these results.
% Based on this result, we assume that even though visual perception can be slow in AR, the perception is as accurate as in VR.
% % RQ - 2
% Interestingly, different from the detection time case, the result with the color alteration condition is not significantly different from the result with the removal condition.
% Similar to the environment cases, we can guess that even though the color visual channel is not good to perceive rapidly, visual confusion does not occur as much as the size alternations.

% \dhk{Similar to the response time results, accuracy results present that it is affected by the visual attention-disrupting methods and the object manipulation methods.
% This measurement means how many times the participants thought the wrong answer was right; Thus, it represents the confusion of detection.
% From the visual attention-disrupting method viewpoint, the turning-60\textdegree method confused participants more than the flickering method.
% But the position and the color of the target object are not related to the result.
% We guess that is because same reason as the upper response time result: detection confusion makes a long response time and low accuracy.
% However, because the position dependency is not found in this accuracy result, we can guess the position effect came from the participant's searching pattern.}

% \dhk{The accuracy results with the manipulation effect show that participants could find the manipulated object more accurately when the object disappeared or its color changed than when the size was changed.
% Similar to the response time results, the color change method has significantly different results compared with the size manipulation methods.
% It is because the accuracy results with other methods are decreased from 3\% to 5\% but with the color change method is not.
% We guess that the same with the response time results, the color perception in the AR environment is not too different from the VR environment.}

% The accuracy of the response (Table~\ref{table_vr_effect_accuracy_result} and right side of Figure~\ref{Response_Time_Plot}) can represent what method makes the viewer confused.
% The main effect of the accuracy is the sight-blocking method (average accuracy for flickering - 98.6\% and turning - 91.8\%, $p$ < .001.)
% As we discussed in the response time section, the visual information in human memory is easily volatilized by a new stimulus.
% This result shows when the visual information changed often (because the participants turned their heads rapidly to find the changed object as fast as possible), the object's attribution in human memory could not be renewed accurately, and it can be strong evidence of the hypothesis 3 (H3): Human memory has a different priority for object attributes.
% Additionally, according to this result, we guess that the often volatilizing of visual information can occur confusion about visual information, which makes the observer thinks the object is changed, but it was not.

\paragraph{\textbf{Timeout Rate}}
Different from the detection rate, this timeout rate results represent the ratio of tasks in which the participants were not able to find the altered object despite their awareness that one of the objects has been altered. This highlights instances where participants experienced difficulty in identifying the altered object within the given time limit (60 seconds).
% ----------- RQ - 1: FoV, VR / AR
Similar to the detection time and rate, the participants find the altered object faster when it is changed inside of FoV in both types of immersive environments.
In VR and AR, the Flickering condition has a significantly lower timeout rate than the Head-Turning condition.
% This result represents that the change blindness effect has easily occurred when the object is changed outside of FoV, and it is a consistent result with the previous change blindness study in VR \cite{martin2023study}, and it supports H1.
This result represents that the change blindness effect has easily occurred when the object is changed outside of FoV, and it supports H1.
Additionally, in AR, the different angles of the Head-Turning conditions do not affect the result.
It is the same with the detection time results and rejects H4; the Head-Turning angle does not affect the Timeout Rate.

% ----------- RQ - 2: Alternation conditions
The Removal condition makes significantly less Timeout Rate than other object alternation conditions only in AR.
However, although the object alternation conditions' effect does not have a significant $p$-value, the order of the timeout rate for each condition in VR is the same within AR.
From this, we can guess that the AR environment has a possibility to reinforce the object alternation condition's effect.

The previous change blindness study in VR \cite{martin2023study} reported the FoV effect on the timeout rate.
It shows consistent results with ours, the alternation that occurred outside of FoV is harder to detect than altered inside of FoV.
However, in that study, they could not find an effect from the type of object alternation.
They did experiments in an environment closer to daily visual experience, which consists of many different shapes of objects that can disturb the participant's attention, and we guess that makes different results from ours.

% This result shows that when the objects are out of the FoV, the observer cannot easily detect the object alternation within the time limit.
% It supports H1; the turning condition makes change detection hard same as the detection time and rate.

% In AR, flickering has a lower timeout than two head-turning conditions.
% And object removal has a lower timeout rate than color alteration, size incrementation, and decrementation.
% These results indicate that the object is moved out from the FoV or not is a dominant point, it is not how much moved out.
% This independency partially rejects H4; the head-turning angle does not affect the timeout rate in the AR environment.
% Different from the result in the VR environment, the removal condition has less timeout rate than other alternation conditions.
% These contrasting results imply that the AR environment amplifies the difficulty of change detection for each condition.
% However, statically, the timeout results do not show a significant difference between VR and AR environments.

% RQ - 1
% Similar to the previous two results, participants could find the altered object faster when it was changed inside of FoV in both types of immersive environments.
% However, the effect of the object alternation condition is only observed in AR significantly, although the order of results is identical in both environments.
% From this, we can guess that the AR environment has a possibility to reinforce the object alternation condition's effect.
% RQ - 2
% Although the object alternation condition's effect in VR is not observed, which is the same as the previous change blindness study in VR, the result with the removal condition in AR is significantly less than the results with others.
% This result depicts that change blindness can occur differently as the type of object alternation.

% \dhk{Additionally, we designed the time limit as 60 seconds, and if the average detection time results with each condition are reached to the limit, this timeout result can be a mixed result between the confusion and
% }
% \dhk{
% Unlike the accuracy, this timeout result shows that the participant could not find the changed object.
% With the flickering method, participants found the target object in almost all tasks (total average timeout ratio is 0.2\%).
% However, with the turning-60\textdegree method, the average is ten times increased to 3.2\%.
% This result represents that when the object is moved out of FoV, the observer cannot detect its change well.
% If the response time result already mentioned above is close to the 60 seconds time limit, the timeout result can be mixed with the long response time. However, the average response time is below 20 seconds, and the timeout ratio with the flickering method is only 0.2\%. These two results show that this timeout result is different cases with just a long response time cases.}

% \dhk{The timeout results show the AR experiment was more difficult than in the VR environment.
% The rate with the flickering is 2\%, and it is 10 times higher than the same method in the VR environment.
% Comparing results between methods is similar to the VR experiment.
% The flickering and removal method has the lowest timeout rate compared to other methods.}

% \textbf{Gazing Time - flickering method:} This result (Table~\ref{table_with_how_long_see_target} and left side of Figure~\ref{Long_Turning_Plot}) shows that even though the participant is watching the changed object, they did not notice it immediately, and this time delay is affected by the object-changing method.
% As already mentioned, the participant took the original and changed scenes in a second.
% However, participants could not notice it while watching the changed object, even the fastest case (disappearing change method) needs more than 5 seconds.
% This result suggests that even though the observer focuses on the object, they need time to cognition that the object is changed.
% Consequently, the strength of the cognition delay effect depends on the object change method, and it supports hypothesis 4 (H4): Even though an observer is focusing on the changing object, they cannot recognize the change immediately.

\paragraph{\textbf{Head-Turning Count}}
This Head-Turning count represents the number of times the participants need to rotate their heads to detect a change that occurs outside of the FoV.
% RQ - 2
In both VR and AR, the Removal condition required the fewest Head-Turning counts to detect change.
This finding indicates the Removal condition is more easily detected with fewer alterations, aligning with the results of detection time and rate. This result supports H1 that the presence or absence of objects is the most memorable aspect of the visual stimulus.

The required counts of other object alternation conditions are similar to each other in VR, but, in AR it is not.
We guess this difference comes from the mixed entities between virtual and real in AR.


% In VR, the participant needs fewer number of alternations to detect change with the removal condition than with other alteration conditions.
% This indicates the removal condition is easily detected with fewer alterations, and it is consistent with the detection time and rate results.
% This result supports H1; the objects' existence is the most easily remembered thing in the visual stimulus.

% In AR, an interaction effect is observed between two turning conditions with different turning angles.

% With both 60$^\circ$ and 30$^\circ$ turning conditions, the removal condition made significantly fewer turning results than the size incrementation and decrementation conditions.
% However, the color alteration condition caused significantly fewer turning count results than the removal condition made with the 30$^\circ$ condition, and it caused larger counts than the decrementation condition with the 60$^\circ$ and the incrementation with the 30$^\circ$.
% Especially, the incrementation with the 60$^\circ$ head-turning condition's result is increased from with the 30$^\circ$ condition's result.
% These results present that the participants tried to remember the objects as many as possible at once, particularly within the 60-turning condition due to the required turning angle.
% Generally, even if the detection time results with the head-turning conditions are longer than the flickering condition, the head-turning counts are fewer than the object's alternations (every 500ms).
% Thus, these results indicate that when the observer has attention carefully, the color can be remembered as much as the object's existence. And it supports H3 and H6.


% The head-turning count with the removal condition is less than other alternations.
% ; it is the same as a result in the VR environment.
% The participants need significantly more times head-turning when the target object is located on the 1st floor than on the 3rd and 4th floors.
% This finding is likely because to the participants' general strategy of searching the structure from top to bottom and on each floor.
% However, this result is guessed due to the participants' general strategy: searching the alternation from top to bottom and on each floor.
% This result strongly supports H6 and the necessity of randomizing the altered object's position in the change blindness experiment.

% RQ - 1 -- X (Only with the turning conditions)

% \dhk{
% Unlike the flicker method, under the turning method condition, the participant has to turn their head to change the object.
% The manipulation method only affects this result; if the target object is manipulated with the removal method, participants had 30\% fewer times head-turning than in other cases.
% It represents that the object's existence is easy to remember, the same reason as the response time result, and because the position is unrelated, we can guess that the participants tried to remember multiple floor objects simultaneously.}


% \dhk{We expected that when the task is difficult, the participant will have more head-turning and we have to worry about fatigue.
% However, according to the result, the head-turning counts in the AR environment are similar to the VR environment.
% Because the response time is increased, this result represents that the participant spent more time without the manipulation, and they had to try remembering more objects at once.
% Consequently, it occurred the interaction effect between the visual attention-disrupting method and the object-manipulation method.
% With the turning 30\textdegree method, the result is the same as the VR experiment. However, with the turning 60\textdegree method, the color change method shows a similar result to the removal method, \textcolor{red}{but the number of head-turning result with the size increased method is decreased 26\%}.
% We guess that when the participant has attention and focus on remembering the object hard, the color attribute can be perceived as similar to its existence.}

% RQ1.How do limited FoVs affect change blindness in VR/AR?
% RQ2.How do different types of object alteration methods affect change blindness in VR/AR?
% RQ3.What are the differences in effects of change blindness between VR and AR?
% \ic{integrated these RQ parts to the above subsections}
% \subsection{Related to RQ1}
% Our findings support H1 and H4 present that when the object is moved out of the FoV, the change blindness phenomenon has occurred stronger.
% However, the distance of how much moved out does not affect it.
% The only matter is whether the observing object moved out of the FoV or not.
% The VR and AR devices we used in this study have different FoVs; the VR device can display objects on all shelves simultaneously, but the AR device can only portray objects on two shelves.
% A combination of this FoV limitation and the finding strategy made a different detection time result affected by the location of the altered object.

% \subsection{Related to RQ2}
% The results support H2 and H3 present the object alternation conditions affect change blindness in both immersive environments.
% The participants could find the removed object most fastly and accurately.
% However, even though the color alternation was the best condition to change detection, the changed details of the object are strongly affected by the visual attention-disrupting conditions and the type of environment(VR/AR).

% \subsection{Related to RQ3}
% As our finding supports H5, although the overall results show the AR environment has the disadvantage of detecting changes, each visual attention-disrupting and object alternation condition presents similar changes.
% The AR environment is mixed with virtual objects and a real background.

\subsection{comparison to the previous studies}
Previous studies in immersive environments designed experiments with different shapes' objects, different backgrounds, and distances~\cite{steinicke2011change, martin2023study}.
This can cause mixed results between the environment and the object's characteristics, such as shape, color, size, and position.
Our experiment is designed to free from that mixing and showed different results.
However, Martin et al. ~\cite{martin2023study} had a different result from ours.
Even though their experiment was conducted in a VR environment, they could not find the effect of object alternation type, and it is not coincident with a previous change blindness study about the alternation type in 2-Dimensional image~\cite{ma2013change}.

% ------------------------ 
% Explain what points are better than previous studies
\dhk{Working}
% 0. Introduction
Change blindness is a conventional research subject for visual perception.
Thus, many researchers have investigated this phenomenon within various environments.
However, most of the studies are investigated within not controlled conditions, such as not identified object shape, unexpected object location, and 
Additionally, many research are conducted within a 2-dimensional display but it is not enough to understand the change blindness in the real world.
% 1. Controlled
%% 1-1. Shape
%%% The visual perception is affected by individual preference, but existing studies didn't consider it.
An individual preference for objects is a dominant property of visual perception.
Thus, identifying the object's shape or at least a theme that can be changed during a task is necessary to investigate the change blindness phenomenon.
However, this identification is hard within an everyday environment, such as a bedroom with furniture, mostly used in the existing studies.
%%% Same shape -> We could exclude the participant's visual preference
In our study, we used objects that have the same modeling.
Consequently, we could exclude the participant's individual visual preferences.
% 1-2. Position (Context)
The position of the objects is one of the other important points for the change blindness study.
An impertinent position will make the participant more focused on that, which can affect the result.

%%% It could be ignored

% 2. Immersive environment
%% 2-1. VR and AR

% 3. Head Turning <- More like with the real world situation (New approach)
%% Flickering <- only for the eye blinking but it is too fast
%% 
% 4. 

% VS all other studies (briefly)

% VS study with 2D images
% 1. Immersive environment
%     i) 3-Dimensional - different perception between 2D and 3D, it occurs different detection rate \cite{korisky2021dimensions}
    % ii) Different memory between immersive and non-immersive system \cite{ventura2019immersive}
% 2. Controlled

% VS study in VR \cite{martin2023study}
% 1. Controlled
    % i) Without any attention disrupting backgrounds

2. Different immersive systems (VR, AR)
    i) Different FoV
    ii) Pure virtual vs Mixed with real(VR, AR)

3. compared each attribution (Color, Size, disappeared)
    i) Investigated with identical shape
    
Additionally, human visual perception and memory are different as the dimension of the visual stimuli \cite{korisky2021dimensions, ventura2019immersive}.

Our study is the first change blindness study that focuses on the properties of changing objects without any attention-disrupting backgrounds.
The related work section mentioned that various change blindness studies were conducted before \cite{}.
However, those studies had too many not controlled visual stimuli such as 
Our experiments present how the attributes of an object (existence, color, and size) affect the change blindness phenomenon.
%

\subsection{Limitation}
Our study is conducted in VR and AR environments and compared results within both environments.
However, due to the limitation of the devices and their FoVs, we could not fully control all variables, such as FoV, interaction techniques (controller in VR and hand gesture in AR), and transparency of virtual objects. Further studies are needed to evaluate the effect of the significantly long period when the altered object is out of the FoV.

% The detection time is a common measurement for the change blindness study.
% However, our result shows that the participant's search strategy dominantly affects the detection time and, particularly, the spatial searching pattern.
% Even though we had spatial balancing to ignore that limitation, that issue was only removed statistically.
Most change blindness studies, even ours, have repeated measuring experiments that ask to find some changed thing.
However, in that procedure, participants will focus on objects and try to remember as much as they can.
Consequently, this kind of study can be just a visual memory test even if the visual working memory is related to the change blindness phenomenon.
% \textbf{Habituation effects}

%\textbf{future work}

==> Contents/Introduction_old.tex <==
% Definition
\section{Introduction}
% \HDY{I think the paragraphs are unnecessarily separated. try to make this section have three or four paragaphs. maybe + 1 more paragraphs summarizing what our contributions are }

% [Change Detection in Virtual Reality]
% Visual stimulus
% Change Detection
% Change Blindness
% What can affect to Change Blindness?
A visual stimulus, a virtual environment created by computer graphics, is the primary component of virtual reality(VR) technology\cite{cummings2016immersive}.
The VR system provides abundant visual information in an immersive environment; then, it can be constrained by the same issues of the human visual system as those in the real world.
The change blindness phenomenon is one of those.
% [About Change blindness]
% \ic{add clear motivation about this research}
Change blindness is a phenomenon that occurs when individuals fail to notice significant changes in their environment, even when those changes are right in front of them \cite{rensink1997see,simons1997change}.
This can occur in a variety of situations, such as when an object is moved or removed from a scene, when a person's appearance is altered, or when an entire scene is transformed.
% [Why it is important]
% Detecting what is changed, how much has or has not been changed, is one of the most necessary capacities to understand a situation as visual information.
% Most people guess that they can figure out the changed things; however, the change blindness phenomenon makes it wrong.
Despite the change detection that overcomes change blindness is possible through training, because it is limited to the specific area, the systematic handling for change blindness is necessary for visual content\cite{gaspar2013change}.
% In the reversible situation, change blindness couldn't be a serious problem. But, in some irreversible situations and requiring rapid decision-making situations such as driving, crime investigation, or military operation, change blindness can be the origin of a huge mistake
Especially in irreversible situations, such as driving, crime investigation, or military operation, even though the operators are already trained, change blindness can cause a serious problem, then decreasing it is significant.\cite{romer2014adolescence, white2010blind, davies2007change, nelson2011change, fitzgerald2016change, divita2004verification}.

% [Virtual Reality + Augmented Reality System for visual perception]
However, research on change blindness in the real world has been limited by the inability to manipulate variables freely, resulting in conditions that do not fully investigate the real-world situation.\cite{simons1999gorillas}
Rather than conducting research on change blindness experiments in the real world, many researchers have investigated this phenomenon under 2D displays with original and modified images.
% In this situation, the advent of head-mounted displays(HMD) for a virtual object has opened a new era of visual perception research under an unlimited number of variables that can be manipulated and controlled within the virtual environment.
In this situation, the advent of head-mounted displays (HMD) for a fully computer-generated 3-dimensional virtual environment has opened a new era of visual perception research under an unlimited number of variables that can be manipulated and controlled within the virtual environment.
% After the VR devices are born, researchers started using them to study visual perception.
Initially, researchers focused on examining the similarities between the visual perception of real-world objects and virtual objects.\cite{kelly2004perception, bingham2001accommodation, giannopoulos2011comparison}
Those results presented that the user experience in virtual environments leads to a heightened focus on visual stimuli while reducing attention to other stimuli\cite{kober2012using}.
As a result, previous studies on virtual environments demonstrate that experiments about visual stimuli are sufficiently meaningful, even though the environment is not entirely identical to those in the real world\cite{wilson2015use}.
For the change blindness studies, the virtual environment served lots of impossible changes in the real world.
The experimental procedures used in studies, such as changing object direction, introducing new objects, or moving a door without producing extraneous noise, are often impractical in the real world.\cite{steinicke2011change, charlton2013driving, suma2011leveraging}
% \ic{add research questions we are trying to attach}
There are many investigations, theories, and experiments to understand change blindness. However, the relation between the strength of change blindness and the object-changing method, or the method to make the sight discontinuity is still unclear.


% [What we will discuss]
In this paper, we conduct a change blindness study in a VR environment with two different sight-blocking methods (flicker and head-turning) and four different object change methods (Disappearing, color change, size increasing, and size decreasing).
We measured how much time the participant needed to find the changing object, how much accurate their detection was, how the eye moved during finding the changed object, and how many times the user turned to find the object.
We utilized the experiment results on the VR environment to examine the impact of two methods ( the object-changing method and the observer sight-blocking method) on the change blindness phenomenon.

% With those results, we investigate the effect of object attributes, sight disruption, and environment on the change blindness phenomenon.

% \ic{highlight the  contributions} \\
% \ic{add the paper organization}

%----------------- How studied(roughly) -----------------
% Making change is a difficult task.
% \HDY{Earlier studies (+ref) evaluated the change blindness by using ... }

% Change blindness study is hard

% Visual display based study cannot present the result in the 3D environment

% Study in a real environment with real objects has limited changing <- hard to investigate what affect on the change blindness

% However, the virtual environment study can have study in 3D environment with unlimited changing.

%----------------- Study with virtual, Augmented reality -----------------
% \HDY{In these days, utilizing VR devices is getting common for a psychological study. 1. cheap, 2. ...}

%---Study in virtual reality
%

%---Study in augmented reality
%Augmented reality environment provide real-virtual mixed visual space.

%

% In addition, the use of Virtual Reality equipment allows researchers to overcome these limitations and manipulate variables in a simulated environment that closely resembles reality in ways that may not be possible in real life.

% The change blindness phenomenon has also been observed in Virtual Reality display systems\cite{steinicke2011change}.

%%%%%%%%%%%%%%% What we will argue in this paper  %%%%%%%%%%%%%%
% In this paper, we introduce two studies (in a virtual reality environment and in an augmented reality environment) with two different sight-blocking methods (flicker and head-turning) and three different object change methods (Disappearing, color change, and size change).
% We measured how much time the participant needs to find the changing object, eye movement during finding the changing object, and how many times the user turned to find the object.
% With those results, we investigate the effect of object attributes, sight disruption, and environment on the change blindness phenomenon.



==> Contents/Result_VR_AR.tex <==
\subsection{VR vs. AR}
% ------------------ Response Time -------------------
Based on our two studies, we provide a comparative analysis of our findings in both VR and AR environments. To ensure a fair comparison, we use consistent Head-Turning conditions of 60 degrees for the comparative analysis.
\begin{table}[ht] 
\caption{\label{table:both_responseTime_sight_manipulation} Statistic results for the response time with the visual attention-disrupting and the object alternation conditions with VR and AR environments.}
\begin{tabular} {m{2.3cm} | m{1.9cm} | m{1cm}| m{0.8cm} | m{0.8cm}}
\toprule 
    {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    Disrupting \texttimes Alternation \texttimes (VR, AR) & {3, 126} & {.334} & {.801} & {.008} \\
    Disrupting \texttimes Alternation  & {3, 126} & {.864}  & {.462} & {.020} \\ 
    Alternation \texttimes (VR, AR)  & {3, 126} & {1.902}  & {.133} & {.043} \\ 
    Disrupting \texttimes (VR, AR)  & {1, 42} & {1.645}  & {.207} & {.038} \\ 
    Disrupting & {1, 42} &  {55.413}  & {\textless .001} & {.569} \\
    Alternation & {3, 126}  & {25.520} & {\textless .001} & {.378} \\
    (VR, AR) & {1, 42}  & {5.051} & {.030} & {.107} \\
    \bottomrule
\end{tabular}
%\vspace{-0.6cm}
\end{table}

\textbf{Detection Time:}
% Any interaction effect is not observed.
% However, three main effects on visual attention-disrupting (F(1,42)=55.413, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.569), object alternation (F(3, 126)=25.520, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.378) and virtual environment (F(1, 42)=5.051, $p$=.030, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.107) conditions are found. 
% The Flickering (M=12.89s, SD=5.38) occurred shorter response time than with the turning - 60\textdegree condition (M=20.17s, SD=7.61, $p$\textless .001); the removal condition (M=13.23s, SD=6.64) occurred shorter response time than with all other object alternation conditions (Color: M=17.05, SD=7.15, $p$\textless .001; Incrementation: M=16.94s, SD=6.87, $p$\textless .001; Decrementation: M=18.91s, SD=8.21, $p$\textless .001). But the decrementation condition has a longer response time than the color ($p$=.008) and incrementation conditions ($p$=.006).
There is a main effect on the immersive environment (F(1, 42)=5.051, $p$=.030, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.107). Overall, VR (M=15.33s, SD=6.41) has a shorter detection time than AR (M=17.74, SD=8.33,$p$=.030), but any interaction effects between the immersive environments and other conditions are not found. 

There is a main effect on visual attention-disrupting (F(1,42)=55.413, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.569). The Flickering (M=12.89s, SD=5.38) occurred shorter response time than with the 60$^\circ$ Head-Turning condition (M=20.17s, SD=7.61, $p$\textless .001).

We also found a main effect on object alternation (F(3, 126)=25.520, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.378). The Removal condition (M=13.23s, SD=6.64) occurred shorter response time than with all other object alternation conditions (Color Alteration: M=17.05, SD=7.15, $p$\textless .001; Size Incrementation: M=16.94s, SD=6.87, $p$\textless .001; Size Decrementation: M=18.91s, SD=8.21, $p$\textless .001). But the Size Decrementation condition has a longer response time than the Color Alteration ($p$=.008) and Size Incrementation conditions ($p$=.006).

% In the VR condition, the result (M=15.33s, SD=6.41) is shorter than in the AR condition (M=17.74, SD=8.33,$p$=.030).
% ------------------ Accuracy -------------------

\begin{table}[ht] %
\caption{\label{table:both_accuracy} Statistic results for the response accuracy with the visual attention-disrupting and the object alternation conditions with VR and AR environments.}
\begin{tabular} {m{2.3cm} | m{1.9cm} | m{1cm}| m{0.8cm} | m{0.8cm}}
\toprule 
    {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    Disrupting \texttimes Alternation \texttimes (VR, AR) & {3, 126} & {.538} & {.657} & {.013} \\
    Disrupting \texttimes Alternation  & {3, 126} & {6.370}  & {\textless .001} & {.132} \\ 
    Alternation \texttimes (VR, AR)  & {3, 126} & {2.244}  & {.086} & {.051} \\ 
    Disrupting \texttimes (VR, AR)  & {1, 42} & {.001}  & {.981} & {.000} \\ 
    Disrupting  & {1, 42} &  {11.235}  & {.002} & {.211} \\
    Alternation & {3, 126}  & {5.199} & {.002} & {.110} \\
    (VR, AR) & {1, 42}  & {.456} & {.503} & {.011} \\
    \bottomrule
\end{tabular}
%\vspace{-0.6cm}
\end{table}

\textbf{Detection Rate:}
The accuracy result does not show any dependency on the type of virtual environment.
However, 
% regardless of the environment, 
an interaction effect (F(3, 126)=6.370, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.132) between the visual attention-disrupting and the object-alternation conditions and two simple effects on the visual attention-disrupting (F(1, 42)=11.235, $p$=.002, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.211) and the object-alternation (F(3, 126)=5.199, $p$=.002, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.110) conditions are found.
In the interaction effect, with the incrementation and decrementation conditions, the flickering method (Incrementation: M=97.7\%, SD=6.35; Decrementation: M=93.9\%, SD=11.7) made more accurate results than the turning - 60$^\circ$ (Incrementation: M=80.5\%, SD=25.9, $p$\textless .001 ; Decrementation: M=83.4\%, SD=25.1, $p$=.015).
The incrementation condition's result (M=97.7\%, SD=6.35) is highly accurate compared to the decrementation condition (M=93.9\%, SD=11.7, $p$=.035) with the flickering condition.
With the turning - 60$^\circ$ condition, the removal (M=94.8\%, SD=12.2) and color (M=91.1\%, SD=18.5) condition made a higher accuracy rate than the incrementation (M=80.5\%, SD=25.9, $p$\textless .001 (Removal),=.003 (Color)) and decrementation (M=83.4\%, SD=25.1, $p$=.002 (Removal),=.009 (Color)) conditions results.
But simply, the flickering condition's accuracy result (M=95.6\%, SD=11.5) is higher than the turning - 60$^\circ$'s result (M=87.4\%, SD=21.9, $p$=.002); the removal condition's result (M=95.7\%, SD=11.4) is higher than the incrementation (M=89.1\%, SD=20.8, $p$=.002) and decrementation (M=88.6\%, SD=20.3, $p$=.001) conditions' results.

% ------------------ Timeout -------------------

\begin{table}[ht] %
\caption{\label{table:both_timeout} Statistic results for the timeout rate result with the visual attention-disrupting and the object alternation conditions with VR and AR environments.}
\begin{tabular} {m{2.3cm} | m{1.9cm} | m{1cm}| m{0.8cm} | m{0.8cm}}
\toprule 
    {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    Disrupting \texttimes Alternation \texttimes (VR, AR) & {3, 126} & {.389} & {.761} & {.009} \\
    Disrupting \texttimes Alternation  & {3, 126} & {3.710}  & {.013} & {.081} \\ 
    Alternation \texttimes (VR, AR)  & {3, 126} & {.972}  & {.408} & {.023} \\ 
    Disrupting \texttimes (VR, AR)  & {1, 42} & {2.908}  & {.096} & {.065} \\ 
    Disrupting  & {1, 42} &  {14.565}  & {\textless .001} & {.257} \\
    Alternation & {3, 126}  & {5.791} & {\textless .001} & {.121} \\
    (VR, AR) & {1, 42}  & {7.265} & {.010} & {.147} \\
    \bottomrule
\end{tabular}
%\vspace{-0.6cm}
\end{table}

\textbf{Timeout:}
This timeout rate presents one interaction effect between the visual attention-disrupting and the object alternation conditions (F(3, 126)=3.710, $p$=.013, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.081) and three simple effects on the visual attention-disrupting condition (F(1, 42)=14.565, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.257), the object alternation condition(F(3, 126)=5.791, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.121), and the virtual environment (F(1, 42)=7.265, $p$=.010, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.147)
In the interaction effect, the flickering condition has less timeout rate than the turning - 60$^\circ$ condition with the color (Flickering: M=1.4\%, SD=5.04; Turning: M=6.8\%, SD=14.1, $p$=.008), incrementation (Flickering: M=2.3\%, SD=7.65; Turning: M=9.5\%, SD=15.7, $p$=.008), and decrementation (Flickering: M=0.45\%, SD=2.98; Turning: M=8.2\%, SD=13.7, $p$\textless .001) conditions. Additionally, the removal condition (M=1.4\%, SD=6.60) has less timeout rate than all other object-alternation conditions (Color: M=6.8\%, SD=14.1, $p$=.012; Incrementation: M=9.5\%, SD=15.7, $p$\textless .001; Decrementation: M=8.2\%, SD=13.7, $p$=.002) with the turning - 60$^\circ$ condition.
In simple effects, less timeout rate results are observed in the VR environment (M=1.7\%, SD=5.98) than in the AR environment (M=5.9\%, SD=13.2, $p$=.010), in the flickering condition (M=1.1\%, SD=5.10) than in the turning - 60$^\circ$ condition (M=6.5\%, SD=13.4, $p$\textless .001), and in the removal condition (M=0.9\%, SD=5.14) than in all the other object-alternation conditions (Color: M=4.1\%, SD=10.9, $p$=.008; Incrementation: M=5.9\%, SD=12.8, $p$\textless .001; Decrementation: M=4.3\%, SD=10.6, $p$=.003).

% ------------------ Head-Turning Count -------------------
\begin{table}[ht] %
\caption{\label{table:both_turning} Statistic results for the head-turning count result with the object alternation conditions with VR and AR environments.}
\begin{tabular} {m{2.3cm} | m{1.9cm} | m{1cm}| m{0.8cm} | m{0.8cm}}
\toprule 
    {\textbf{Factor}} & {\textbf{$DOF$}}  & {\textbf{$F$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\ \midrule
    Alternation \texttimes (VR, AR)  & {3, 126} & {2.778}  & {.044} & {.062} \\ 
    Alternation & {3, 126}  & {11.832} & {\textless .001} & {.220} \\
    (VR, AR) & {1, 42}  & {.728} & {.398} & {.017} \\
    \bottomrule
\end{tabular}
%\vspace{-0.6cm}
\end{table}

\textbf{Head-Turning Count:}
There is an interaction effect between the object-alternation and the virtual environment conditions (F(3, 126)=2.778, $p$=.044, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.062). A simple effect on the object-alternation condition (F(3, 126)=11.832, $p$\textless .001, $\eta$\textsubscript{$p$}\textsuperscript{$2$}=.220) is found. In AR, the removal condition (M=4.27, SD=1.58) made less number of head-turning results than the incrementation (M=5.53, SD=2.54, $p$=.018) and decrementation (M=6.71, SD=2.43, $p$\textless .001) conditions.  And the color (M=4.96, SD=2.38, $p$=.002) and incrementation (M=5.53, SD=2.54, .017) conditions have fewer numbers than the decrementation (M=6.71, SD=2.43). However, in the VR environment, the removal condition (M=4.56, SD=1.47) occurred less number of head-turning than all others (Color: M=6.66, SD=3.42, $p$\textless .001; Incrementation: M=6.01, SD=3.02, $p$=.002; Decrementation: M=6.37, SD=2.37, $p$\textless .001) but others are not significantly different from each other.
Overall, the removal condition (M=4.18, SD=1.53) made less number of head-turning than all other object-alternation conditions (Color: M=5.81, SD=3.04, $p$=.001; Incrementation: M=5.77, SD=2.80, $p$\textless .001; Decrementation: M=6.54, SD=2.40, $p$\textless .001). And the incrementation condition (M=5.77, SD=2.80) made a result less than the decrementation condition (M=6.54, SD=2.40, $p$=.026).



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> old_files/README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> old_files/Related_Work.tex <==
\section{Related Work}
% % [The origin]
% The coherence theory suggests a mechanism for detecting changes in visual stimuli whereby an observer compares visual representations before and after a change.\cite{rensink2002change}
% These representations are created by the observer's attention and are stored in human visual memory, which has limited capacity.\cite{hollingworth2004constructing}
% As a result, visual attention and memory are considered as a dominant role in the occurrence of change blindness.\cite{simons2005change,levin1997failure,rensink2000visual, rensink2002failure}

\subsection{Change Blindness}
% \HDY{add what the earlier studies' results are. clarify what are known and tackle what are unknown and challenging. based on the them clarify what we are going to do in this paper}

% [Study for the change blindness itself]
After the first discovery of change blindness, this impressive phenomenon was investigated in many conditions.
%   [Gorilla]
One of the famous change blindness studies is "Gorillas in our midst."\cite{simons1999gorillas}
This study presented that even though the participants focused on the video, participants could not remember, or figure out the unexpected stranger (a human under an umbrella or wearing a full-body gorilla suit) who passed through the center of the video.
The percentage of participants who noticed the stranger depends on the transparency of the video, the type of stranger (wearing a gorilla suit or under the umbrella), and the difficulty of the mission that made participants focus on the video.
This study showed that the unexpected event can not be perceived, even the event that occurred at the center of vision, if the viewer focuses on the other.
%   [Failure to detect changes to attended objects in motion pictures] \cite{levin1997failure}

The change blindness phenomenon occurs even the observer doesn't focus on other things.
In a study, people can not notice a human changing in the real-world scene video.
Even though the participants attended to the video as much as they could remember details of clothing, the environment, and actor movements, they remained unaware of substituting one actor with another\cite{levin1997failure}.
Similarly, when the individuals in front of the observer were changed during communication, they couldn't notice the change\cite{simons1998failure}.


However, these kinds of real-world situation studies couldn't investigate what variables affect the strength of change blindness and why the change blindness phenomenon occurred.
Therefore, Researchers conducted a controlled investigation of change blindness in static images to facilitate a controlled experimental environment.

%   [Studies in the static images]
%[Failures of Retrieval and Comparison Constrain Change Detection in Natural Scenes]
Studying with static images can handle every visual stimulus that couldn't be in real-world study.
One of the most frequently used experimental methods for studying change blindness involves presenting two-dimensional static images, which are repeated alternately and require participants to identify changes between them.
Through this study, researchers could improve the understanding of the human visual perception process and the origin of change blindness\cite{landman2003large, lamme2003visual, hollingworth2003failures}.
However, the characteristics of the visual stimulus, such as its dimension, can result in differences in human perception\cite{korisky2021dimensions}.
%       [Partially converted stereoscopic images and the effects on visual attention and memory] \cite{kim2015partially}
But the change blindness phenomenon is still occurring in the different dimension images (2D, 3D, and partial 3D)s \cite{kim2015partially}.

\subsection{Change Blindness in Virtual Reality}
%   [Studies in the 3D]
Although the study with the displayed image can provide a wide range of visual stimuli, it still has limitations for the change blindness study.
%       [stereoscopic scenes] \cite{steinicke2011change}
% However, within the virtual reality environment, there is a new era of change blindness study.
However, within the virtual environment, the change blindness study can be improved one step further.
Steinicke et al. investigated change blindness phenomena in three stereoscopic display systems (Active Stereoscopic Workbench, Passive Back-Projection Wall, and Head-Mounted Display). This study used the response time(change detection time) to evaluate the strength of the change blindness effect. Even though there are differences depending on the display systems and detail conditions, the change blindness phenomenon has occurred in every type of display system.

%       [driving] \cite{charlton2013driving}

Not only the virtual reality provides a new possibility to the change blindness study but also, the change blindness can make progress for virtual reality.
%       [leverage the virtual space] \cite{suma2010exploiting, suma2011leveraging}
The change blindness phenomenon can solve one of the major problems of the virtual reality system. Most VR devices couldn't provide a larger virtual space than real tracking space. However, a leverage technique using change blindness can solve this limitation. This technique makes users walk around the same small space but feels they are in a huge virtual space with many rooms by changing the direction of the room's door when the door is out of their sight.
Interestingly, most of the participants couldn't notice that change and they had an illusion such as they are really in a huge virtual space\cite{suma2010exploiting, suma2011leveraging}.

In this way, change blindness and virtual reality technology can provide mutually benefit each other.
However, the factors that can weaken or strengthen change blindness in virtual reality remain unexplored area.
In this paper, we will argue about what can reinforce the change blindness phenomenon and what can undermine it.
%       [Change Blindness in AR] \cite{kitamura2019monocular}


% %%%%%%%%%%%%% About Change Blindness phenomenon itself %%%%%%%%%%%%%
% % Definition of Change Blindness - Change blindness is defined as the failure to detect when a change is made to a visual stimulus (Simons and Levin, 1997).
% Near the 1990s, several studies presented the change blindness phenomenon in natural and artificial scenes\cite{blackmore1995richness,grimes1996failure,rensink1997see}.

% % When occur? -  eye blink (O’Regan et al., 2000), saccadic eye movement (Grimes, 1996; McConkie and Currie, 1996), screen flicker (Rensink et al., 1997), a cut or pan in a motion picture (Simons, 1996; Levin and Simons, 1997), when the local visual transient produced by a change coincides with multiple local transients at other locations(mud splashes) (O’Regan et al., 1999).

% Many kinds of situations that the change blindness emerged were reported: saccadic eye movement\cite{grimes1996failure,mcconkie1996visual}, discontinuity of visual scene\cite{rensink1997see}, and eye blinking\cite{kevin2000picture}.

% Unexpected changing makes the change blindness phenomenon more strongly\cite{williams2000detecting, triesch2003you}.

% %----------------- Change methods -----------------
% In the pursuit of understanding change blindness, researchers have conducted experiments utilizing various object-changing methods and different object-changing timing.
% Change a person who had a conversation with the participant to someone else during sight is blocked by disturbance\cite{simons1998failure}.
% Changing is synchronized with saccadic eye movements or blinks\cite{henderson1999role, kevin2000picture}.
% Changing object during the image has sinusoidal oscillations\cite{schofield2006oscillatory}.
% Flicker\cite{rensink1997see}

% %%%%%%%%%%%%% About Change Blindness study in 2D display %%%%%%%%%%%%%
% Most of the cases, change blindness studies used a computer display and compared two similar but little different images.
% With real-world image studies.
% With basic shapes studies.
%     Color changes with moving
% Comparing the change blindness effect between on the real world and on screen viewing \cite{attwood2018comparison}
% Change blindness difference between 2-dimensional image and 3-dimensional image \cite{kim2015partially}.


% %%%%%%%%%%%%% About Change Blindness study in others(immersive environment, Virtual Reality) %%%%%%%%%%%%%
% Studies for extending the user's perceived virtual space used the change blindness phenomenon to reach their goal\cite{suma2010exploiting, suma2011leveraging, langbehn2018blink}.
% Study for the driver detection of a change in the well-knowing environment\cite{charlton2013driving}.
% Comparing a study between a few types of stereoscopic scenes but it was a study with real-world images \cite{steinicke2011change}.

% Despite the potential of virtual reality environments for studying change blindness, it wasn't investigated yet.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Physical Behavior (related with attention)

% including limitations on memory capacity, links between attention and awareness

% Study about change detection
% There are many studies that have investigated understanding human change detection\cite{rensink2002change}.

%What is important for change detection - Attention
% There are many parameters that affect change detection, but consequently, those things are focused on the observer's attention\cite{rensink1997see}.

%Used change blindness test - response time - for investigating visual attention and memory
% Study for the visual attention and memory investigation of converted images used the change blindness\cite{kim2015partially}.


%Study about change blindness
%When it occurred, examples
%Why it occurred
    %Coherence theory
    %[]
% Awareness, attention,
%limited memory capacity
%Study about awareness, attention, perception

%Study about human perception in 3D images - Using Change blindness test for investigating visual attention and memory
%[Partially converted stereoscopic images and the effects on visual attention and memory]
%Change blindness experiment for investigate the effect of partially converted 3D images on a subject's concentration and memory.
%Change blindness task makes consideration to human cognitive characteristics with respect to the observation of 3D images.
%In VR
%Study about user awareness, attention, and perception in VR (X)

%Study about Change Blindness in VR (X)

%Flicker -> Visual => Blocking => Visual
%Turning -> VIsual => Blocking + visual is spatialy changed + [physical behavior] => Visual

% Testable - Change blindness is a testable phenomenon that can be used to investigate the nature of visual representations in different conditions (Simons and Rensink, 2005).

% \HDY{\subsection{VR as a Psychological(?) Research Tool}}


==> old_files/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

